AG-CVG: Coverage Planning with a Mobile Recharging UGV and an Energy-Constrained UAV

In this paper, we present an approach for coverage path planning for a team of an energy-constrained Unmanned Aerial Vehicle (UAV) and an Unmanned Ground Vehicle (UGV). Both the UAV and the UGV have predefined areas that they have to cover. The goal is to perform complete coverage by both robots while minimizing the coverage time. The UGV can also serve as a mobile recharging station. The UAV and UGV need to occasionally rendezvous for recharging. We propose a heuristic method to address this NP-Hard planning problem. Our approach involves initially determining coverage paths without factoring in energy constraints. Subsequently, we cluster segments of these paths and employ graph matching to assign UAV clusters to UGV clusters for efficient recharging management. We perform numerical analysis on real-world coverage applications and show that compared with a greedy approach our method reduces rendezvous overhead on average by 11.33%. We demonstrate proof-of-concept with a team of a VOXL m500 drone and a Clearpath Jackal ground vehicle, providing a complete system from the offline algorithm to the field execution.

==> reviews/iros_2023.tex <==
\section{Reviewer 1}

The paper studies a planning method to coordinate multiple
ground and aerial vehicle for coverage problem. The added
twist to the problem is the fact that the aerial vehicle
must rendezvous with the ground vehicle to recharge so that
it can execute the entire mission.  The authors propose a
heuristic algorithm to solve the planning problem, and
provide some experimental result.

The topic seems to be of importance to the field, and the
paper is overall well organized, but there are a few
concerns as discussed below.

-Clarity of the technical approach

The authors mention that “only one of the robots (UAV)
needs to take the rendezvous route.”  Does this mean that
there is only one UAV in the team? Furthermore, it is
unclear whether this is an assumption on the problem, or
the consequence of the proposed algorithm.

The definition of “pass” is not very clear to the reader. 
Specifically, it is unclear whether the pass means a
piece-wise linear segment, or the collection of those
segments. The relationship between “passes” and “path
segment” is unclear.

The formulation of the maximum-matching problem is not very
clear.	How is the bipartite graph constructed? Is this
based on the overlap in the regions in xy plane?  Also,
maximum matching finds the largest cardinality for
matching, so it is unclear what t\_max means and how it is
computed.

These details need to be clarified in order for the result
of this paper to be reproducible.


-Significance of the results and experiments

The value of field study is unclear in the context of the
proposed work. It can be seen that the vehicles execute way
point navigation as specified by the algorithm, but what
does this demonstrate/validate?  

The 7\% improvement against a greedy method does not seem to
be significant, given that the greedy method uses much less
computational load.

-Other comment

The duration of the submitted video is 1 min. 52 sec.,
which violates the 1 min. limit of the video.

Some texts are going outside of the “blocks” in Fig. 2.


\section{Reviewer 2}
This paper deals with path planning for UGV and UAV that
have a work-time constraint necessary for recharging.
Authors proposed the algorism for AG-Cvg and experimentally
confirmed. Experiments are performed in actual outside and
wide environments. We think the better results are
obtained, however, we think we need more detailed
verifications of your experimental condition and data in
order to confirm your ideas.

Experimental results shown in Fig.4 and Fig. 6 may be
unclear. If we see the experimental results in Fig.4 to
compare AG-Cvg and Greedy, we cannot catch which is
performed better. 

In P4 right L6, and conclusion, you write “AG-Cvg
outperforms on average by at least 7% on the other
scenarios”, however, caption in Fig.5 say “it is lower by
at least 10% on the other senarios”, which describes is
right or that causes my misunderstandings? And moreover,
the difference seems too small, we cannot know and judge
this difference causes effectiveness of your algorithm or
another factors. We think we need more detailed explanation
and another experimental data comparison.


\section{Reviewer 3}

This paper proposes an approach for coverage planning for a
team of UAV and UGV - AG-Cvg algorithm.
The UAV is energy-constrained and the UGV is recharging
station for the UAV.
This planning problem is known to be NP-hard. A heuristic
method to solve this coupled planning problem is proposed:
A)find coverage paths without considering energy
constraints,  
B)cluster segments of the coverage paths
C)apply graph matching to assign UAV clusters to UGV
clusters to handle recharging
The planning pipeline of AG-Cvg is implemented and
evaluated by simulation and field test using DJI drone.
In the result of the pipeline reduces 7\% the rendezvous
overhead than Greedy approach.

1) The proposed AG-CVg algorithm does not use the
information of maximum speed of UAV or UGV. Don't they
affect the result of the pipeline?
For example, if the UGV is much faster than UAV, the
coverage path of UGV supposed to be longer than UAV.

2) The meaning of Fig.3 is hard to understand. Explanation
is needed. 

3) In main text, referring to Fig.1,2,and 3 are missing.

4) No information of UGV in explanation of field
deployment. 

\section{Video Comments:}

\begin{itemize}
    \item The developed AG-Cvg is illustrated. It is better if the charging motion is included. 
\item The video exceeded the 1 min limit.  It was 1 min 52 sec.
\item We can get the results of computer simulation, however, we
cannot find the field experiments (both UAV and UGV are
moved together along authors proposed algorithm). 
\end{itemize}

==> sections/reviews.tex <==
\textbf{Review 4: }
The authors provided a lot of work for this study with
theoretical reasoning and experimental validation, which is
a good work, but there are still some problems, and I would
like to make four main suggestions.

1. This paper lacks ablation experiments. In the
experimental section, the focus is on describing the
implementation of the whole function and the comparison
with the greedy method, but the impact of the core module
on the whole task is not analyzed, which lacks a certain
degree of persuasiveness.

2. The quality of the images in the article needs to be
improved. Several images in the article are not clear,
e.g., Figures 3 and 6. The clarity of the images affects
the rigor of the article, so please revise as appropriate.

3. Lack of data support in the real-world experiment part.
The paper does not provide a specific data list or running
trajectory monitoring in the real-world experiment part,
and only has some pictures to illustrate, so it is
recommended to supplement the data verification.

4. Air-ground communication problem for this article. This
work involves the cooperation of air-ground equipment, but
the article does not show a description of the construction
of the communication system, please add a description of
how the communication problem between the two equipment is
solved.

Finally, we thank the authors for their contribution to the
field and hope that the authors will be better able to
extend and improve this work afterwards. 

\textbf{Review 7: }

The paper is well written and presented piece of work. The
paper discusses a coverage path planning solution for a
team of an energy-constrained Unmanned Aerial Vehicle (UAV)
and an Unmanned Ground Vehicle (UGV). 

The choice of a boustrophedon decomposition coverage
planning
solution may render the overall framework inflexible in
certain non-regular mapping scenarios resulting in cases
where either the UGV or UAV are idle or not being used. 

Although, the authors provide a procedure of handling such
scenarios, the inherent adaptability of the framework can
be significantly improved with a flexible primary coverage
solution. Perhaps, directly optimizing for the vertices
locations of the bipartite graph under bounded vertices
constraints could be an more flexible approach.
Furthermore, such a solution would also lend its more
robustness in presences of realistic flight conditions.

Furthermore, the simulation comparison provided with the
greedy method seems under-discussed. A claim of improved
performance over the greedy algorithm needs more
stimulative studies than 11 scenarios, I would recommend at
least 50 scenarios . Moreover, the use of a fractional
coverage trajectory requirements may not provide an
holistic perspective. The authors should also consider
adding data associated with the average number of charging
instances, total mission times, total idle run times of
either the UAV or UGV as compared to the greedy algorithm. 

\textbf{Video Comment:}
- The work is well thought out and the entire system
framework is well designed 
- More emphasis on the experimental study should be provided
with additional text explanations. 

\textbf{Associate Editor:}
- The article's main concept(s)
A big area of research in mobile robotics is the area
coverage with heterogeneous multi-robot systems. Area
coverage can address search and rescue missions, area
patrolling, and area mapping and has a dependency on doing
it with efficiency under coverage path planning.
In this work, the authors present a coverage planning with
a team of UGV and UAV, where the UAV is energy-constrained
and the UGV might work as a recharging platform.
Both robots are assigned an area to cover, and the main
goal is to accomplish complete coverage with both robots
while minimizing the coverage time. A second goal is due to
the UAV battery limitations, the UGV can work as a recharge
station and both robots need to rendezvous for the
recharging manoeuvre.
Both robots have a predefined area that needs to be covered
in the minimum coverage time by choosing the best path
planning, and taking into account the UAV battery
constraint and possible rendezvous with UGV to recharge.
Recharge missions increase the coverage time due to
rendezvous travel time and idle recharging time.



The work is compared to state-of-the-art and achieves
similar results but at a higher prediction speed test.
 
- Overall Comment
In overall, 
An interesting topic, that deals with area path planning
coverage with UAV and UGV while having the possibility of
the UGV recharging the UAV (rendezvous missions).
The UAV energy constraint might raise some global objective
conflicts, as it is important to balance between the main
goal of total coverage and the rendezvous and recharge
missions.
Recharging a UAV takes time, therefore it would be
beneficial if the UGV could continue the mission after the
UAV docking, while this one is still charging on top of it.
From the simulations and real scenario testing, both UAV
and UGV are stopped during the UAV charging phase.
The authors propose an Air-Ground Coverage Path Planning
Algorithm (AG-Cvg) that starts by creating coverage paths
ignoring the energy issues. Then, segments the paths
(boustrophedon decomposition coverage planning BCD) and
uses graph matching methods to match UAV and UGV path
clusters and minimize the travel distances to rendezvous.
The AG-Cvg method was compared to the Greedy approach in
eleven different regions and size scenarios. 

- Weak and Strong points

Strengths
- The paper addresses an important topic –
Multi-robots area coverage;
- Heterogeneous team of UAV and UGV
collaborating in area coverage and power transfer;
- A heuristic approach to deal with an
NP-Hard motion planning problem;

Weakness
- Simple boustrophedon path planning and
graph matching for coverage planning – with the novelty
being the UAV-UGV recharging maneuver;
- It is no novelty or a major scientific
contribution – for a leading conference such as ICRA;

There are several issues identified by the reviewers that
have to be addressed and clarified. Please look at the
review comments to improve the paper. The authors are
encouraged to improve the paper and future work following
the reviewers' comments.
